Improved Topological Preservation in 3D Axon Segmentation and Centerline Detection using Geometric Assessment-driven Topological Smoothing (GATS)

Automated axon tracing via fully supervised learning requires large amounts of 3D brain imagery, which is time consuming and laborious to obtain. It also requires expertise. Thus, there is a need for more efficient segmentation and centerline detection techniques to use in conjunction with automated annotation tools. Topology-preserving methods ensure that segmented components maintain geometric connectivity, which is especially meaningful for applications where volumetric data is used, and these methods often make use of morphological thinning algorithms as the thinned outputs can be useful for both segmentation and centerline detection of curvilinear structures. Current morphological thinning approaches used in conjunction with topology-preserving methods are prone to over-thinning and require manual configuration of hyperparameters. We propose an automated approach for morphological smoothing using geometric assessment of the radius of tubular structures in brain microscopy volumes, and apply average pooling to prevent over-thinning. We use this approach to formulate a loss function, which we call Geo-metric Assessment-driven Topological Smoothing loss, or GATS. Our approach increased segmentation and center-line detection evaluation metrics by 2%-5% across multiple datasets, and improved the Betti error rates by 9%. Our ablation study showed that geometric assessment of tubular structures achieved higher segmentation and centerline detection scores, and using average pooling for morphological smoothing in place of thinning algorithms reduced the Betti errors. We observed increased topological preservation during automated annotation of 3D axons volumes from models trained with GATS.

==> tables/table5.tex <==

\setlength{\tabcolsep}{2pt}
\npdecimalsign{.}
\nprounddigits{2}

\begin{table}[ht]\centering
    \caption{\textbf{DS2 Affine Rotation Transformation Sensitivity}} 
    \label{tab:sens_table}
    \begin{NiceTabular}{c  |c | c | c | c | c| c }
    \hline
       \thead{\textbf{Model}} & \textbf{Dice $\uparrow$} & \textbf{clDice $\uparrow$} & \textbf{$\rho$-Dice $\uparrow$} & \textbf{Adj. Rand $\uparrow$} & \textbf{$\beta_{0}$ Error $\downarrow$} & \textbf{$\beta_{1}$ Error $\downarrow$} \\ \hline \hline
        
        % not _2 models
        
        \textit{clDice (Set 1)} & 0.7880   \text{\small$\pm$}  0.0140 & 0.6890   \text{\small$\pm$}  0.0270 & 0.7750   \text{\small$\pm$}  0.0300 & 0.5760  \text{\small$\pm$}  0.0270 & 0.1270   \text{\small$\pm$}  0.0310 & 0.1510   \text{\small$\pm$}  0.0170  \\ \cline{2-7}

        \textit{clDice (Set 2)} & 0.2360 \text{\small$\pm$} 0.0554 & 0.0315 \text{\small$\pm$} 0.0159 & 0.0901 \text{\small$\pm$} 0.0318 & $-$0.0053 \text{\small$\pm$} 0.0017 & 0.8076 \text{\small$\pm$} 0.1591 & 0.5619 \text{\small$\pm$} 0.0594 \\ \cline{2-7}

       \textit{clDice (Set 3)} & 0.1010 \text{\small$\pm$} 0.1592 & 0.0718 \text{\small$\pm$} 0.0555 & 0.1147 \text{\small$\pm$} 0.0612 & 0.0002 \text{\small$\pm$} 0.0077 & 0.2317 \text{\small$\pm$} 0.3270 & 0.6015 \text{\small$\pm$} 0.0928 \\ \cline{2-7}

        \textit{GATS (N=10, Set 1)} & 0.7321 \text{\small$\pm$} 0.0065 & 0.5699 \text{\small$\pm$} 0.0149 & 0.6418 \text{\small$\pm$} 0.0163 & 0.4637 \text{\small$\pm$} 0.0129 & 0.0461 \text{\small$\pm$} 0.0076 & 0.1023 \text{\small$\pm$} 0.0094 \\ \cline{2-7}

        \textit{GATS (N=10, Set 2)} & 0.8029 \text{\small$\pm$} 0.0068 & 0.7146 \text{\small$\pm$} 0.0156 & 0.8060 \text{\small$\pm$} 0.0156 & 0.6052 \text{\small$\pm$} 0.0135 & 0.0472 \text{\small$\pm$} 0.0100 & 0.0956 \text{\small$\pm$} 0.0135 \\ \cline{2-7}

        \textit{GATS (N=10, Set 3)} & 0.8029 \text{\small$\pm$} 0.0062 & 0.7149 \text{\small$\pm$} 0.0122 & 0.7997 \text{\small$\pm$} 0.0159 & 0.6052 \text{\small$\pm$} 0.0124 & 0.0565 \text{\small$\pm$} 0.0192 & 0.1081 \text{\small$\pm$} 0.0220 \\ \hline

        
    \end{NiceTabular}
\end{table}

==> tables/table6.tex <==
\setlength{\tabcolsep}{2pt}
\npdecimalsign{.}
\nprounddigits{3}

\begin{table*}[ht]\centering
    \caption{\textbf{Efficient Channel Attention (ECA) and Triplet Attention (TA) on 3D Residual UNets. Mean and standard deviation evaluated on the test set of Dataset 1 (DS1) and Dataset 2 (DS2) across 10 trials. For clDice: $\alpha=0.65, k=3$, GASK and GATS both use MPR, for which N=10, GASK uses soft-skeletonization, GATS uses topological smoothing (TS). For TS: k=5 for DS1, k=3 for DS2.} } 
    \label{tab:att_table}
    \small
    \begin{NiceTabular}{ccc |c | c | c | c | c | c }
    \hline
    \textbf{Attention} & \textbf{Dataset} & \thead{\textbf{Model}} & \textbf{Dice $\uparrow$} & \textbf{clDice $\uparrow$} & \textbf{$\rho$-Dice $\uparrow$} & \textbf{Adj. Rand $\uparrow$} & \textbf{$\beta_{0}$ Error $\downarrow$} & \textbf{$\beta_{1}$ Error $\downarrow$} \\ \hline \hline
    %%%%%%%%%%%%%%%%%%ECA%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     ~ & ~ & clDice & 0.7951 $\pm$ 0.0070 & 0.7665 $\pm$ 0.0153 & 0.7521 $\pm$ 0.0184 & 0.5887 $\pm$ 0.0139 & 0.3572 $\pm$ 0.0176 & 0.0803 $\pm$ 0.0092 \\
     ECA & DS1 & GASK & 0.7824 $\pm$ 0.0138 & 0.7287 $\pm$ 0.0457 & 0.7296 $\pm$ 0.0429 & 0.5632 $\pm$ 0.0277 & 0.3284 $\pm$ 0.0218 & 0.0698 $\pm$ 0.0147 \\
     ~ & ~ & GATS & 0.8031 $\pm$ 0.0084 & 0.7471 $\pm$ 0.0194 & 0.7713 $\pm$ 0.0205 & 0.6047 $\pm$ 0.0167 & 0.3223 $\pm$ 0.0250 & 0.0682 $\pm$ 0.0074 \\ \cline{3-9}
     
     ~ & ~ & clDice & 0.7491 $\pm$ 0.0067 & 0.6046 $\pm$ 0.0155 & 0.6808 $\pm$ 0.0164 & 0.4976 $\pm$ 0.0133 & 0.0638 $\pm$ 0.0164 & 0.1199 $\pm$ 0.0115 \\
     ~ & DS2 & GASK & 0.5924 $\pm$ 0.0139 & 0.6500 $\pm$ 0.0201 & 0.7449 $\pm$ 0.0137 & 0.1905 $\pm$ 0.0258 & 0.0602 $\pm$ 0.0259 & 0.4541 $\pm$ 0.0135 \\
      ~ & ~ & GATS & 0.7331 $\pm$ 0.0114 & 0.5696 $\pm$ 0.0247 & 0.6424 $\pm$ 0.0264 & 0.4657 $\pm$ 0.0227 & 0.0508 $\pm$ 0.0092 & 0.1040 $\pm$ 0.0119 \\

    \hline \hline
    %%%%%%%%%%%%%%%%%%TA%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    ~ & ~ & clDice & 0.7970 $\pm$ 0.0076  & 0.7650 $\pm$ 0.0189  & 0.7537 $\pm$ 0.0197 & 0.5924 $\pm$ 0.0152 & 0.3611 $\pm$ 0.0207 & 0.0817 $\pm$ 0.0112 \\
    TA & DS1 & GASK   & 0.7892 $\pm$ 0.0124 & 0.7399 $\pm$ 0.0332 & 0.7348 $\pm$ 0.0344 & 0.5769 $\pm$ 0.0248 & 0.3085 $\pm$ 0.0334 & 0.0618 $\pm$ 0.0115 \\
    ~ & ~ & GATS & 0.8058 $\pm$ 0.0050 & 0.7515 $\pm$ 0.0067 & 0.7701 $\pm$ 0.0133 & 0.6100 $\pm$ 0.0100 & 0.3076 $\pm$ 0.0424 & 0.0627 $\pm$ 0.0064 \\ \cline{3-9}
    
    ~ & ~ & clDice & 0.7423 $\pm$ 0.0115 & 0.5912 $\pm$ 0.0241 & 0.6673 $\pm$ 0.0268 & 0.4840 $\pm$ 0.0229 & 0.0674 $\pm$ 0.0127 & 0.1268 $\pm$ 0.0110 \\
    ~ & DS2 & GASK & 0.6059 $\pm$ 0.0273 & 0.6486 $\pm$ 0.0261 & 0.7437 $\pm$ 0.0152 & 0.2165 $\pm$ 0.0520 & 0.0606 $\pm$ 0.0237 & 0.4450 $\pm$ 0.0280 \\
    ~ & ~ & GATS & 0.7325 $\pm$ 0.0089 & 0.5707 $\pm$ 0.0203 & 0.6443 $\pm$ 0.0205 & 0.4645 $\pm$ 0.0177 & 0.0455 $\pm$ 0.0070 & 0.1028 $\pm$ 0.0080 \\
    \hline \hline

    \end{NiceTabular}
\end{table*}

==> takeout.tex <==
%intro:
Particularly for biomedical images with curvilinear structures, even a generalizable model such as Segment Anything (SAM) requires fine-tuning and adaptation \cite{MedSAM, zeroshot}. The need to fine-tune a foundation model like SAM for curvilinear structure segmentation highlights the need for developing and refining topology-preserving methods. Furthermore, 

Moreover, a dearth of annotated training data can be compensated for by using self-supervised learning methods \cite{klinghoffer2020selfsupervised, tang2022self, shamsi2023}. The assumed drawback of training only on labeled data is that learned feature representations may preclude variations in a structure's topology that were not captured by the annotations, and as such self-supervised learning tasks especially designed for curvilinear structure segmentation may be useful \cite{klinghoffer2020selfsupervised}.

We observed that some of our models which were trained with skeletonization algorithms had degraded performance if the data were preprocessed using certain affine rotation transformations. This observation aligns with the fact that 

\paragraph{Deep Distance Transform (DDT)} The distance transform is an operator that produces an input-sized distance map where each value is the distance from each foreground pixel/voxel to the foreground boundary \cite{DDT}. For volumetric inputs each tubular structure voxel is assigned a value, using an Euclidean distance transform, which is the nearest distance from that voxel to the tubular structure surface \cite{DDT}. The DDT model trains a multi-task deep network to predict both the segmentation mask and distance map of a curvilinear structure, and as such the predicted distance map encodes the geometry of the curvilinear structure. One head of the DDT model does voxel-wise classification for segmentation with a weighted cross-entropy loss function, while the other head predicts a scale class for tubular structure voxels using a distance loss function. While the DDT model does not explicitly promise topology-preservation, we use a multi-headed approach in this study using a Cascading 3D UNet and our method. Multi-headed approaches have been used for 3D axon segmentation and centerline detection previously, but used topology-preservation via a skeletonization method \cite{pollack2022axon}. 

 The third trial consisted of removing GATS and using a Dice loss with inputs from the Topological Smoothing algorithm applied to the segmentation prediction and target (, or just the segmentation prediction and target to compute the objective function.

 This section also covers topology-preserving methods for curvilinear structure segmentation using loss function-based methods which can be used within any deep learning architecture, or deep learning architectures where any objective function may be used.

\subsubsection{Loss-based Methods}
Topology-preserving loss functions for curvilinear structure segmentation can be formulated using inputs from algorithms that transform or engineer features of image inputs; they can be used in any deep learning architecture of interest as long as the image input is correct for the method.

\subsubsection{Deep Learning-based Methods}
Deep learning-based methods for curvilinear structure segmentation use training data for learning feature representations that can be used for precise and accurate segmentation. 

\paragraph{Joint Topology-preserving and Feature-refinement Network (JTFN)} The JTFN is a model for learning global topology and refined features using iterative feedback learning \cite{JFTN}. The JTFN architecture includes two novel modules: the Feature Interactive Module (FIM) and the Gated Attentive Unit (GAU). After an initial convolution on the input, the input is passed to a GAU block which forms a feedback loop using the segmentation prediction and boundary detection to refine features using context and spatial awareness. The GAU is situated between the skip connections of each corresponding encoder and decoder \cite{JFTN}, while the FIM blocks are used as reciprocative decoders between segmentation and boundary detection. The feedback learning strategy is based on accumulating a total loss from a given \emph{T} iterations of forward passes, and then performs backpropagation. The JTFN model was evaluated on different datasets using F1 scores, and measures of Correctness, Completeness and Quality that compared the similarity between predicted skeletons and ground truth within a certain threshold (set to 2). In comparison to other methods for curvilinear structure segmentation, JTFN scores the best 22 out of 24 times \cite{JFTN}. The JTFN appears to be a good candidate for axon tracing and centerline detection, which was not shown in the original paper. Per our knowledge, the JTFN is not currently adapted for voxel-wise segmentation.

\paragraph{Deep Distance Transform (DDT)} The distance transform is an operator that produces an input-sized distance map where each value is the distance from each foreground pixel/voxel to the foreground boundary \cite{DDT}. For volumetric inputs each tubular structure voxel is assigned a value, using an Euclidean distance transform, which is the nearest distance from that voxel to the tubular structure surface \cite{DDT}. The DDT model trains a multi-task deep network to predict both the segmentation mask and distance map of a curvilinear structure, and as such the predicted distance map encodes the geometry of the curvilinear structure. One head of the DDT model does voxel-wise classification for segmentation with a weighted cross-entropy loss function, while the other head predicts a scale class for tubular structure voxels using a distance loss function. While the DDT model does not explicitly promise topology-preservation, we use a multi-headed approach in this study using a Cascading 3D UNet and our method. Multi-headed approaches have been used for 3D axon segmentation and centerline detection previously, but used topology-preservation via a skeletonization method \cite{pollack2022axon}.

\paragraph{
Hu \cite{hu2022structureaware} uses 4-adjacency for the foreground (FG) pixels and 8-adjacency for the background (BG) pixels for 2D images, while 6-adjacency for FG and 26-adjacency for BG for 3D volumes. A pixel or a voxel is a simple point if it can be flipped from FG-to-BG or from BG-to-FG without changing the topology of the image \cite{BERTRAND19941003}.} 

ablation:
Without MPR and \emph{k}=5, models achieved greater centerline detection scores relative to no attention versions of clDice for both DS1 and DS2 datasets: 0.78 $\pm$ 0.02 and 0.72 $\pm$ 0.01 for DS1 and DS2, respectively. 

However, GATS without attention with MPR determined \emph{k}=3 has a greater centerline detection score. 

Taking the MPR results together with the results for GATS models without attention, we observe that the random sampling, data-driven approach of \emph{MPR} seems to acquire a better parameter for the number of iterations required for topological. The Dice and adjusted Rand scores for each dataset seemed to increase indicating better segmentation. The Betti errors for on DS1 showed an increase indicating worsened topological preservation. For DS2 only Betti 0 increased while Betti 1 decreased.

Replacing soft thinning with a general thinning algorithm driven by \emph{MPR} resulted in lower clDice metrics for DS1 and DS2, while all other metrics increased including the Betti errors. This is consistent with our initial trials where another skeletonization over-thinned given inputs. For DS2 using a Dice loss to train the model improved Dice, ARI, $\beta_1$ but not clDice or $\beta_0$ versus the GATS variant, indicating better segmentation but poorer centerline detection. The DS1 scores for the Dice loss did not beat the scores for the GATS variant for any metric. The GATS attention models seem the most performant for segmentation and centerline detection for DS1 and DS2.

discussion
As mentioned, our research aims to maximize topology-preservation of
segmented axons from 3D volumes and to use that to automatically an-
notate unannotated brain imagery. Volumetric brain imagery data is less publicly available and so for teams working on curvilinear structure segmentation of axon-like data, that presents a challenge. The Janelia dataset is the closest set of similar data for our use case. Moreover, our most successful experimental trials have been with some flavor of a UNet architecture, and we find that as another limiting factor as other deep learning architectures that we have tested require more data for robust performance for both segmentation and centerline detection. Future directions for this work will focus on fine-tuning an adapter for Segment Anything that can be used for fine and small curvilinear structure segmentation, while including morphological thinning-based methods like clDice and GAST in foundation model adapters. Our study indicates that skeletonization methods that use differentiable operations for morphological thinning may produce output that are not robust to affine rotation transformations, and 2) 3D brain imagery data may be prone to over-thinning without the use of methods like average pooling-based thinning that can prevent that. For the first remark, there is evidence that skeletons produce via Euclidean distance transforms are relatively robust to rotations \cite{DDT}.

 We evaluated the trials of Warping loss that did complete and found that the centerline detection results of Warping loss were unstable, and so we modified Warping loss to utilise a discrete cosine transform and inputs of soft-skeletonization for homotopic warping, but the performance gains on DS1 were still minimal compared to the increase in training time (Supplementary Material).

\subsection{Skeletal Warping: Discrete Cosine Transform Variant of Warping Loss}
Our experiments with the Warping loss \cite{hu2022structureaware} showed an increase in training time for DS1 to  $\sim$34 hours for 10 trials with Warping loss versus  $\sim$4 hours for clDice,  $\sim$8 hours for GATS (N=10) or $\sim$6 hours for GATS (N=4). To expedite training time we formulated a novel variant of the Warping loss that applies a discrete cosine transform to the soft-skeletonized inputs of the prediction and the target image, and finds critical points of the skeletal topology as described previously; see Homotopic Warping under section \ref{sec:rel}: Related Literature. The evaluation metrics on DS1 of the Skeletal Warping loss are similar to the GATS SCA (N=10) loss, with an improvement in training time on DS1 by $\sim$10 hours. Visually, the Skeletal Warping loss produces better segmentation and centerline detection results, indicating that a hybrid loss function that utilizes homotopic warping for finding critical points of the skeletal topology is promising for topology preservation. However more experiments are required for testing on different datasets and improvements in training time.
